Adaptive Ensemble Biomolecular Simulations at Scale

Recent advances in both theory and methods have created opportunities to simulate biomolecular processes more efficiently using adaptive ensemble simulations. Ensemble-based simulations are used widely to compute a number of individual simulation trajectories and analyze statistics across them. Adaptive ensemble simulations offer a further level of sophistication and flexibility by enabling high-level algorithms to control simulations based on intermediate results. Novel high-level algorithms require sophisticated approaches to utilize the intermediate data during runtime. Thus, there is a need for scalable software systems to support adaptive ensemble-based applications. We describe the operations in executing adaptive workflows, classify different types of adaptations, and describe challenges in implementing them in software tools. We enhance Ensemble Toolkit (EnTK) -- an ensemble execution system -- to support the scalable execution of adaptive workflows on HPC systems, and characterize the adaptation overhead in EnTK. We implement two high-level adaptive ensemble algorithms -- expanded ensemble and Markov state modeling, and execute upto $2^{12}$ ensemble members, on thousands of cores on three distinct HPC platforms. We highlight scientific advantages enabled by the novel capabilities of our approach. To the best of our knowledge, this is the first attempt at describing and implementing multiple adaptive ensemble workflows using a common conceptual and implementation framework.

==> comp_motivation.tex <==
\jhanote{This section needs two parts: The first part of why adaptive
workflows are difficult. Then why EnTK based approach is the right
approach/solution. The latter point in turn is comprised of why its the right
solution for adaptivity and ensemble based applications}

% It is becoming increasingly clear that the application of ensemble simulation
% strategies on state-of-the-art computational facilities has an unparalleled
% potential to permit accurate simulations of the largest, most challenging, and
% generally most biologically relevant, bio-molecular systems. Recently, there
% has been a proliferation of simulation strategies that introduce adaptivity in
% the application workflow, both in order to increase sampling efficiency and
% reduce manual footprint.

There are several hurdles in supporting such adaptive applications on 
traditional HPC systems. HPC systems are traditionally built for static 
applications that consist of a single execution kernel utilizing 100-1000 
compute nodes concurrently. Adaptive EBAs present two challenges:  
(i) supporting the execution of multiple tasks with various dependencies on
HPCs (ii) supporting the ability to capture and analyze intermediate results, 
express changes to the task graph during runtime, and execute tasks of the 
adapted task graph.


% \begin{itemize}

%   \item HPC systems are traditionally built for single, monolithic and static
% applications that utilize 100-1000 compute nodes concurrently and thus
% leave little possibilities for adaptive applications.
%   \item 
% \end{itemize}

% Hence, there is need for tools that enable both the expression and execution
% of adaptive applications.


% \begin{itemize}
% \item HPC systems traditionally designed for one monolithic application and 
% static execution. We break both monolithic model and static execution
% \item Express Adaptivity. No consistent way or form to do so.
% \item Need runtime system to do so. Approaches and tradeoffs (scale, 
% flexibility etc).
% \end{itemize}

When workflow systems were originally conceived, there were no well
established abstractions and “resource management” concepts such as Pilot-Jobs
or standardized access-layers. Thus, the first generation of workflow systems
needed to be end-to-end integrated systems supporting everything from
application development/interfaces, dynamic resource management and access to
heterogeneous middleware layers. At the turn of the century, there was a
proliferation of workflow systems each requiring finer grained support for
advanced task and resource management.

% A partial analysis of DAGMan~\cite{???} and attempts to separate the resource
% access layer from DAGMan functionality shows that the absence of well defined
% interface had important consequences. The absence of general purpose
% scientific languages such as Python motivated the need for specific /
% customized workflow languages and possibly specific workflow programming
% models. There were a few ``important'' workflows that were worth the
% significant efforts in integrating with workflow systems. For example, out of
% 60 workflows that LIGO needs/has, exactly one is ``workflow system
% enabled''~\cite{??}. In general the number of workflows that need supporting
% have increased, but the effort to adapt existing workflow solutions has
% remained high.

% Due to the increasing richness in the user applications and demands on the 
% workflow systems, in this project, we discuss the \entk framework that takes a 
% building blocks approach over an end-to-end system. In this approach, each of 
% the block components have their respective functions and the application 
% requirements of the user can be created using a combination of these components.
%  There are multiple reasons on why this approach can be truly beneficial.

% \begin{description}
% \item \textbf{Proliferation of domain specific workflow systems:} There are a 
% number of "smaller" domain specific workflow systems (DSWS) developed that are 
% not as resourceful as the workflow systems developed by big projects. Although 
% each of the DSWS differ in the overall science problem being solved, they have 
% many overlapping core requirements in resource, task and data management. A 
% generic approach where these functionalities are the responsibilities of a 
% domain-independent components could be beneficial. This isolates the science 
% problem being solved from the resource, task, data management complexities that 
% are not necessarily of the domain scientist's interests. 

% \item \textbf{Last mile customization often has significant upstream 
% consequences:} The ''point of integration'' between capabilities is not always 
% uniform. Early customization of the software frameworks can be disadvantageous 
% as this prevents reuse of optimized solutions from or to other similar problems 
% and requires considerable effort in making modifications. Domain specific 
% customization should be done as last as possible in the software framework. 
% This requires providing building blocks so the users can focus on the science 
% problem, as opposed to all teams repeating and developing the same features 
% poorly.These building blocks are needed by tool developers and 
% application/domain scientists alike.

% \item \textbf{Engineering for Performance:} Performance is a multi-dimensional 
% parameter; thus there are many directions/dimensions in which the framework 
% needs to be tuned. It is non-trivial to tune the entire stack of the framework 
% along specific parameters. Building Block approach provides modularity. In a 
% workflow management system not all layers of the stack equally contribute to 
% performance; closer to the system level the more critical from a performance 
% point-of-view. It would be more useful to be able to tune each of the layers 
% of the stack based on performance requirements that the entire stack.
% This is not to say that we shouldn’t have end-to-end workflow systems. They 
% retain a role. However, there are two classes of users that are not being served 
% with the current set of monolithic workflow tools and systems: (i) Workflow 
% system and tool developers, and (ii) domain scientists interested only in the 
% science questions.
% The vision as a consequence of well-defined, designed and implemented 
% building blocks, developing workflows will be closer to python programming 
% using scientific libraries. Ideally each building blocks can be provided as 
% library, where these libraries have well defined interfaces and semantics but 
% each library is engineered for performance on platforms. This will prevent 
% workflow vendor lock-in and rigidity in programming models.
% \end{description}

% Many of which “grow” or “evolve” as the science
% advances (thus reiterating the importance of end-user “development”). The effort
% to “integrate” the remaining 59 workflows of LIGO is arguably uneconomical.


% \subsubsection{Challenges of the building blocks approach?}

% \begin{itemize}
% \item Performance versus generality: Can adequate performance be achieved whilst
% aiming for components that are general and extensible to be used by multiple
% distinct applications and tools.

% \item Integration complexity: A multi-component design approach has the challenge of 

% \item Impedance mismatch: Similarly there is a risk of “functional gaps”..

% \end{itemize}



